Depth Reconstruction with Neural Signed Distance Fields in Structured Light Systems

We introduce a novel depth estimation technique for multi-frame structured light setups using neural implicit representations of 3D space. Our approach employs a neural signed distance field (SDF), trained through self-supervised differentiable rendering. Unlike passive vision, where joint estimation of radiance and geometry fields is necessary, we capitalize on known radiance fields from projected patterns in structured light systems. This enables isolated optimization of the geometry field, ensuring convergence and network efficacy with fixed device positioning. To enhance geometric fidelity, we incorporate an additional color loss based on object surfaces during training. Real-world experiments demonstrate our method's superiority in geometric performance for few-shot scenarios, while achieving comparable results with increased pattern availability.

==> chapters/backup.tex <==
\begin{table*}
  \centering
  \begin{tabular}{@{}cccccccccccccccccc@{}}
    \toprule
    \multirow{2}*{Num.} & \multirow{2}*{Methods} & \multicolumn{3}{c}{Scene 0} & \multicolumn{3}{c}{Scene 1} & \multicolumn{3}{c}{Scene 2} & \multicolumn{3}{c}{Scene 3} \\
    ~ & ~ & o(1.0) & o(5.0) & avg & o(1.0) & o(5.0) & avg & o(1.0) & o(5.0) & avg & o(1.0) & o(5.0) & avg \\
    \midrule
    \multirow{4}*{7} & Naive~\cite{posdamer1982surface} & 83.84 & 25.65 & 3.572 & 77.85 & 11.13 & 6.033 & 82.40 & 22.82 & 4.262 & 82.78 & 23.53 & 4.035\\
    ~ & NeRF~\cite{niemeyer2022regnerf} & 78.04 & 26.04 & 13.644 & 81.76 & 45.48 & 21.493 & 67.99 & 23.14 & 12.622 & 68.90 & 20.84 & 11.986 \\
    ~ & NeuS~\cite{wang2021neus} & 100.00 & 100.00 & 700.540 & 100.00 & 100.00 & 644.709 & 100.00 & 100.00 & 718.422 & 100.00 & 100.00 & 720.956 \\
    ~ & Ours & \textbf{58.91} & \textbf{3.74} & \textbf{2.517} & \textbf{66.85} & \textbf{26.16} & \textbf{16.273} & \textbf{59.08} & \textbf{11.59} & \textbf{8.670} & \textbf{55.14} & \textbf{12.23} & \textbf{12.584}\\
    \hline
    \multirow{4}*{6} & Naive~\cite{posdamer1982surface} & 92.50 & 62.48 & 7.066 & 90.64 & 51.18 & 8.716 & 92.14 & 59.75 & 7.853 & 92.12 & 60.24 & 7.630\\
    ~ & NeRF~\cite{niemeyer2022regnerf} & 74.12 & 29.10 & 16.666 & 84.11 & 46.44 & 19.476 & 67.30 & 23.79 & 10.901 & 64.96 & 20.07 & 8.832 \\
    ~ & NeuS~\cite{wang2021neus} & 100.00 & 100.00 & 700.461 & 100.00 & 100.00 & 644.278 & 100.00 & 100.00 & 718.146 & 100.00 & 100.00 & 720.648\\
    ~ & Ours & \textbf{65.15} & \textbf{5.86} & \textbf{3.906} & \textbf{80.53} & \textbf{30.38} & \textbf{16.816} & \textbf{72.20} & \textbf{15.57} & \textbf{9.979} & \textbf{59.53} & \textbf{11.55} & \textbf{12.357}\\
    \hline
    \multirow{4}*{5} & Naive~\cite{posdamer1982surface} & 95.91 & 80.94 & 13.960 & 94.59 & 74.68 & 13.826 & 95.95 & 79.97 & 14.951 & 95.61 & 79.57 & 14.676 \\
    ~ & NeRF~\cite{niemeyer2022regnerf} & 77.16 & 36.88 & 16.059 & 84.68 & 48.14 & 19.360 & 73.10 & 26.03 & 9.910 & 71.39 & 22.81 & 9.810 \\
    ~ & NeuS~\cite{wang2021neus}  & 100.00 & 100.00 & 700.550 & 100.00 & 100.00 & 644.281 & 100.00 & 100.00 & 718.176 & 100.00 & 100.00 & 720.677\\
    ~ & Ours & \textbf{65.87} & \textbf{12.69} & \textbf{4.307} & \textbf{76.12} & \textbf{33.30} & \textbf{17.071} & \textbf{56.30} & \textbf{16.43} & \textbf{10.732} & \textbf{73.02} & \textbf{17.21} & \textbf{9.081}\\
    \hline
    \multirow{4}*{4} & Naive~\cite{posdamer1982surface} & 98.15 & 90.71 & 28.199 & 97.58 & 87.60 & 24.443 & 97.97 & 89.85 & 29.269 & 98.05 & 90.11 & 29.216\\
    ~ & NeRF~\cite{niemeyer2022regnerf} & 86.80 & 56.81 & 22.514 & 91.13 & 62.76 & 31.432 & 84.37 & 45.43 & 14.840 & 81.65 & 36.89 & 17.019 \\
    ~ & NeuS~\cite{wang2021neus} & 100.00 & 100.00 & 700.630 & 100.00 & 100.00 & 644.433 & 100.00 & 100.00 & 718.229 & 100.00 & 100.00 & 720.734\\
    ~ & Ours & \textbf{74.34} & \textbf{30.19} & \textbf{8.304} & \textbf{80.87} & \textbf{43.17} & \textbf{20.282} & \textbf{69.56} & \textbf{24.62} & \textbf{8.582} & \textbf{71.72} & \textbf{22.12} & \textbf{7.337}\\
    \hline
    \multirow{4}*{3} & Naive~\cite{posdamer1982surface} & 99.06 & 95.25 & 56.596 & 98.81 & 93.74 & 45.419 & 99.00 & 94.89 & 58.713 & 99.01 & 95.09 & 58.938\\
    ~ & NeRF~\cite{niemeyer2022regnerf} & 95.50 & 83.68 & 43.286 & 96.65 & 85.81 & 49.108 & 96.35 & 82.76 & 32.862 & 94.41 & 75.41 & 33.430\\
    ~ & NeuS~\cite{wang2021neus} & 100.00 & 100.00 & 700.452 & 100.00 & 100.00 & 644.261 & 100.00 & 100.00 & 718.270 & 100.00 & 100.00 & 720.774\\
    ~ & Ours & \textbf{93.99} & \textbf{73.80} & \textbf{26.877} & \textbf{93.02} & \textbf{74.24} & \textbf{24.825} & \textbf{91.39} & \textbf{68.19} & \textbf{21.170} & \textbf{89.08} & \textbf{58.94} & \textbf{19.118}\\
    \bottomrule
  \end{tabular}
  \caption{The experiment results with the gray code pattern projected. "Num." indicates that how many digital numbers we used for gray code.}
  \label{tab:orderexp}
\end{table*}

\begin{table*}
  \centering
  \begin{tabular}{@{}cccccccccccccccccc@{}}
    \toprule
    \multirow{2}*{Ind.} & \multirow{2}*{Methods} & \multicolumn{3}{c}{Scene 0} & \multicolumn{3}{c}{Scene 1} & \multicolumn{3}{c}{Scene 2} & \multicolumn{3}{c}{Scene 3} \\
    ~ & ~ & o(1.0) & o(5.0) & avg & o(1.0) & o(5.0) & avg & o(1.0) & o(5.0) & avg & o(1.0) & o(5.0) & avg \\
    \midrule % 12345
    \multirow{3}*{23456} & NeRF~\cite{niemeyer2022regnerf} & 78.19 & 35.69 & 19.785 & 82.66 & 43.76 & 21.188 & 76.65 & 24.31 & 12.374 & 64.21 & 20.48 & 7.830 \\
    ~ & NeuS~\cite{wang2021neus} & 100.00 & 100.00 & 700.533 & 100.00 & 100.00 & 644.396 & 100.00 & 100.00 & 718.301 & 100.00 & 100.00 & 720.806\\
    ~ & Ours & \textbf{67.61} & \textbf{5.79} & \textbf{3.986} & \textbf{71.98} & \textbf{28.77} & \textbf{16.864} & \textbf{58.88} & \textbf{17.16} & \textbf{9.548} & \textbf{57.73} & \textbf{13.08} & \textbf{9.959}\\
    \hline % 01346
    \multirow{3}*{12457} & NeRF~\cite{niemeyer2022regnerf} & 76.15 & 29.74 & 17.477 & 84.09 & 54.44 & 27.051 & 71.85 & 30.75 & 16.651 & 68.48 & 26.89 & 14.293\\
    ~ & NeuS~\cite{wang2021neus} & 100.00 & 100.00 & 700.402 & 100.00 & 100.00 & 643.851 & 100.00 & 100.00 & 718.320 & 100.00 & 100.00 & 720.825\\
    ~ & Ours & \textbf{52.76} & \textbf{6.66} & \textbf{5.888} & \textbf{66.94} & \textbf{30.23} & \textbf{19.833} & \textbf{69.22} & \textbf{16.12} & \textbf{7.909} & \textbf{64.65} & \textbf{12.60} & \textbf{9.909}\\
    \hline % 0235
    \multirow{3}*{1346} & NeRF~\cite{niemeyer2022regnerf} & 77.32 & 31.05 & 14.861 & 81.98 & 47.79 & 19.933 & 76.74 & 26.54 & 10.096 & 71.36 & 21.83 & 12.342\\
    ~ & NeuS~\cite{wang2021neus} & 100.00 & 100.00 & 700.454 & 100.00 & 100.00 & 643.984 & 100.00 & 100.00 & 718.324 & 100.00 & 100.00 & 720.829 \\
    ~ & Ours & \textbf{64.79} & \textbf{8.79} & \textbf{3.740} & \textbf{70.48} & \textbf{28.00} & \textbf{17.065} & \textbf{56.47} & \textbf{13.85} & \textbf{7.722} & \textbf{66.64} & \textbf{13.50} & \textbf{11.640}\\
    \hline % 1346
    \multirow{3}*{2457} & NeRF~\cite{niemeyer2022regnerf} & 79.29 & 26.32 & 14.206 & 81.72 & 51.25 & 27.556 & 68.12 & 26.35 & 13.608 & 65.45 & 21.52 & 9.801\\
    ~ & NeuS~\cite{wang2021neus} & 100.00 & 100.00 & 700.618 & 100.00 & 100.00 & 644.582 & 100.00 & 100.00 & 718.314 & 100.00 & 100.00 & 720.819\\
    ~ & Ours & \textbf{69.61} & \textbf{5.81} & \textbf{3.651} & \textbf{63.87} & \textbf{24.31} & \textbf{14.740} & \textbf{66.93} & \textbf{12.05} & \textbf{8.647} & \textbf{56.35} & \textbf{11.17} & \textbf{5.445}\\
    \bottomrule
  \end{tabular}
  \caption{The experiment results for randomly selected patterns. We use the index of patterns to mark out which patterns we selected for evaluation.}
  \label{tab:disorderexp}
\end{table*}
